Approximate Generalized Matching: $f$-Factors and $f$-Edge Covers

In this paper we present linear time approximation schemes for several generalized matching problems on nonbipartite graphs. Our results include $O_\epsilon(m)$-time algorithms for $(1-\epsilon)$-maximum weight $f$-factor and $(1+\epsilon)$-approximate minimum weight $f$-edge cover. As a byproduct, we also obtain direct algorithms for the exact cardinality versions of these problems running in $O(m\sqrt{f(V)})$ time. The technical contributions of this work include an efficient method for maintaining {\em relaxed complementary slackness} in generalized matching problems and approximation-preserving reductions between the $f$-factor and $f$-edge cover problems.

==> conclusion.tex <==
\section{Conclusion and Open Problems}\label{sect:conclusion}

We give the first almost linear time approximation schemes for both \textsc{maximum weight $f$-matching} and \textsc{minimum weight $f$-edge cover problem}.  This result generalizes the algorithm by Duan and Pettie~\cite{DP14} for approximate weighted matching problems. We also establish approximation preserving reductions between the two problem inside the primal-dual framework for weighted matching, showing that any approximation algorithm that also produces an approximately optimal dual solution to one problem can be transformed to an approximation algorithm to the other problem. 

We demonstrate that with the appropriate generalization of key concepts such as blossoms and augmenting paths, we can derive direct algorithm for generalized matching problems from its corresponding version for $1$-matching, instead of relying on inefficient reductions. Thus, it is natural to ask whether other algorithm for $1$-matching, such as~\cite{DuanPS14} can be generalized to $f$-matching.

Another key open problem is whether we can obtain linear dependency in graph size for our algorithm, i.e. eliminating the factor $\alpha(m, n)$ in the time complexity. The key challenge here is to give a union find data structure for maintaining blossoms on a dynamic tree as specified in Section~\ref{sec:aug-walk}. 
